Regularized Data Programming with Automated Bayesian Prior Selection

The cost of manual data labeling can be a significant obstacle in supervised learning. Data programming (DP) offers a weakly supervised solution for training dataset creation, wherein the outputs of user-defined programmatic labeling functions (LFs) are reconciled through unsupervised learning. However, DP can fail to outperform an unweighted majority vote in some scenarios, including low-data contexts. This work introduces a Bayesian extension of classical DP that mitigates failures of unsupervised learning by augmenting the DP objective with regularization terms. Regularized learning is achieved through maximum a posteriori estimation with informative priors. Majority vote is proposed as a proxy signal for automated prior parameter selection. Results suggest that regularized DP improves performance relative to maximum likelihood and majority voting, confers greater interpretability, and bolsters performance in low-data regimes.

==> figures_tex/schematic.tex <==
% LF train
$\begin{bmatrix}
    \lambda_0 & \lambda_1 & \lambda_2 \\
    0 & 0 & 1 \\
    0 & 0 & 1 \\
    0 & -1 & 1 \\
    \vdots & \vdots & \vdots
\end{bmatrix}$

% LF test
$\begin{bmatrix}
    \lambda_0 & \lambda_1 & \lambda_2 \\
    0 & 0 & 1 \\
    0 & 0 & -1 \\
    0 & 0 & 1 \\
    \vdots & \vdots & \vdots
\end{bmatrix}$


\begin{table}[]
    \centering
    \begin{tabular}{|l l c|}
    \hline
        \textsc{PubMed ID} & \textsc{Manuscript title} & $y$ \\
    \hline
       33485387 & Time-course single-cell RNA sequencing... & 1 \\
       31852401 & Longitudinal RNA-seq analysis of the... & -1 \\
       30527648 & Time series analysis of gene changes and... & -1 \\
       $\vdots$ & $\vdots$ & $\vdots$ \\
    \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:df_train}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{|l l c|}
    \hline
        \textsc{PubMed ID} & \textsc{Manuscript title} & $y$ \\
    \hline
       13677474 & Temporal progression of gene expression... & 1 \\
        31997507 & Temporal profile of HEV RNA... & -1 \\
        19147844 & Dynamic gene expression is required for... & -1 \\
       $\vdots$ & $\vdots$ & $\vdots$ \\
    \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:df_test}
\end{table}

% Train
$\begin{bmatrix}
    \hat{y} \\
    1 \\
    1 \\
    -1 \\
    \vdots
\end{bmatrix}$

% Test
$\begin{bmatrix}
    \hat{y} \\
    1 \\
    -1 \\
    1 \\
    \vdots 
\end{bmatrix}$

\begin{table}[]
    \centering
    \begin{tabular}{|l|}
    \hline
         • Priors over labels $\hat{y}$ \\
         • Priors over LF accuracies $\alpha$ \\
         • Priors over LF coverages $\beta$ \\
         \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:priors}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{|c|}
    \hline
    {\textsc{Train DP}} \\
    \textsc{generative model} \\
         \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:priors}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{|c|}
    \hline
    {\textsc{Apply}} \\
    \textsc{trained model} \\
         \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:priors}
\end{table}


    \begin{table}
    \centering
    \begin{tabular}{|l|}
         \hline
         \textsc{Labeling function} \\
         \hline
         $\lambda_0$: \texttt{exclude\_organism} \\
         $\lambda_1$: \texttt{include\_terms} \\
         $\lambda_2$: \texttt{exclude\_terms} \\
         \hline
    \end{tabular}
    \label{tab:lfs}
\end{table}

Apply labeling functions to textual data

\textbf{1.} \\
\textbf{2.} \\
\textbf{3.} \\
\textbf{4.} \\
\textbf{5.} \\
\textbf{6.} \\

$\mathbf{P}(\hat{y})$


$\mathbf{P}(\alpha)$


$\mathbf{P}(\beta)$

